Bose-Einstein condensation: Twenty years after

The aim of this introductory article is two-fold. First, we aim to offer a general introduction to the theme of Bose-Einstein condensates, and briefly discuss the evolution of a number of relevant research directions during the last two decades. Second, we introduce and present the articles that appear in this Special Volume of Romanian Reports in Physics celebrating the conclusion of the second decade since the experimental creation of Bose-Einstein condensation in ultracold gases of alkali-metal atoms.

==> hyphenJournals.tex <==
\hyphenation{pro-per-ties dif-fe-ren-ti-al re-con-si-der-ed Clifford com-pac-ti-fi-ca-tions co-ho-mo-lo-gy de-fi-ni-tions in-fi-ni-te-si-mal sa-tis-fies a-u-xi-li-a-ry Princeton ge-ne-ra-li-zes ge-ne-ra-li-zed ge-ne-ra-li-za-tion ge-ne-ra-li-za-tions mo-di-fi-ca-tion re-du-ci-bi-li-ty pre-sen-ce e-qui-va-lent a-na-ly-ti-cal li-ne-a-ri-zed gra-vi-ty res-tric-tions re-de-fi-ni-tions ge-ne-ra-tors coun-ter-terms Einstein se-pa-ra-te-ly ge-o-me-tri-cal phy-si-cal con-ti-nu-a-tion par-ti-cu-lar ge-o-me-tric se-con-da-ry ca-no-ni-cal ge-ne-rat-ing ge-ne-ra-ted ge-ne-ra-te si-mi-la-ri-ties e-vi-den-ce res-pec-ti-ve-ly po-la-ri-za-tion cor-res-pond-ing e-ner-gy ga-la-xies ga-la-xy sym-me-tric in-te-res-ting cor-res-pond-ing o-pe-ra-tors o-pe-ra-tor Riemann va-ri-ous va-cu-um se-pa-ra-bi-li-ty cha-rac-te-rized cha-rac-te-ri-zec cha-rac-te-ri-za-tion re-a-li-za-tion co-e-xist-ing re-la-ti-vi-ty af-fi-ni-ty ma-xi-mal or-tho-go-nal Budapest ex-pe-ri-ment res-pon-se to-po-lo-gi-cal an-ti-sym-me-tric ma-ni-fold me-thod me-
thods na-no-struc-tu-re na-no-struc-tu-res a-na-ly-sis Qua-si-re-so-nant e-vinced re-so-nan-ce re-so-nant dy-na-mics con-ti-nu-um pa-ra-me-ter pa-ra-me-ters de-ve-lop-ment non-li-ne-a-ri-ties va-ni-shes va-nish res-pect ge-ne-ral non-li-ne-ar re-la-ti-ve-ly ho-lo-gra-phy pro-per-ty li-ne-ar re-la-ti-ve par-ti-cu-lar-ly cha-rac-ter con-fi-gu-ra-tion su-per-a-sym-me-tric in-di-vi-du-al ne-gli-gi-ble me-cha-ni-cal con-si-der-ed ap-pro-xi-ma-tion ap-pro-xi-ma-tions Fredholm e-le-ment mo-di-fy mo-di-fied Coulomb Schroedinger Einstein Perelemov tra-vel-ling ci-vi-li-zed hie-rar-chy tran-sac-tion tran-sac-tions pro-ba-bi-li-ty se-cond se-cond-ly Se-cond-ly Heisenberg se-mi-nal Mottelson re-co-ve-ry pro-blem li-mit li-mi-ted re-le-vant exist a-ve-rage e-va-lu-ate con-ti-nu-a-tion}
\hyphenation{ty-pi-cal ap-pro-xi-ma-te-ly ex-pe-ri-men-tal res-pon-si-ble gra-vi-ta-tio-nal si-mi-la-ri-ty de-ve-loped ge-ne-ral-ly}

==> rrp_mathdefs.tex <==
  %This file contains a hopefully ever growing collection of command shortcuts and even new LaTeX commands (especially for math mode),
% that are currently in use and accepted by Romanian Journal of Physics.
%Last modified: 07/2011 (dd/mm/yyyy)

%Environment and general command shortcuts
\providecommand{\beq}[1][\@empty]{\def\@ttoken{#1}\begin{equation}\dbg@ut{\@ttoken}\ifx\@empty#1 \else\label{#1}\fi}
\newcommand{\eeq}{\end{equation}}
\newcommand{\beqn}{\begin{equation*}}
\newcommand{\eeqn}{\end{equation*}}

%elliptic Jacobi functions
\DeclareMathOperator{\sn}{sn}
\DeclareMathOperator{\cn}{cn}
\DeclareMathOperator{\dn}{dn}

%Mathematical operators and various symbols
\DeclareMathOperator{\ddiv}{div}
\DeclareMathOperator{\grad}{grad}
% Hyperbolic functions
\DeclareMathOperator{\artanh}{artanh}
\DeclareMathOperator{\sech}{sech}
\DeclareMathOperator{\cosech}{csch}
\DeclareMathOperator{\cosec}{cosec}
\DeclareMathOperator{\sgn}{sgn}
\newcommand{\eps}{\ensuremath{\varepsilon}}
\newcommand{\cc}{\ifmmode\mathrm{cc.\;}\else\textrm{cc.~}\fi}
\newcommand{\ict}{\ifmmode\mathcal{C}\else\texttt{C}\fi}
\providecommand{\pd}{\ensuremath{\partial}}
\providecommand{\dd}{\ensuremath{\mathrm{d}}}
\providecommand{\id}{\ensuremath{\;\mathrm{d}}}

%bras and kets
\providecommand{\bra}[1]{\ensuremath{\left<#1\right|}}
\providecommand{\ket}[1]{\ensuremath{\left|#1\right>}}
%the \braket command is thought to be the matrix element of operator #1 for state #2 (left) and state #3 (right)
\providecommand{\braket}[3]{\ensuremath{\left<#2|#1|#3\right>}}

%Commands for multiple indexes around a central token #1
%The names derive from "front up-down, back up-down" of #1 (it better be read as "left up-down, right up-down") indicating 
%the order in which indexes are passed starting with #2 (left-up or front-up). The only cool stuff about these commands is 
%that it diminishes the space between up-down left indexes and the following token.
\newcommand{\fudbud}[5]{{\!\;}^{#2}_{#3}\!\!#1^{#4}_{#5}}
\newcommand{\fubu}[3]{{\!\;}^{#2}\!\!#1^{#3}}
\newcommand{\fdbd}[3]{{\!\;}_{#2}\!\!#1_{#3}}
\newcommand{\fdbu}[3]{{\!\;}_{#2}\!#1^{#3}}
\newcommand{\fubd}[3]{{\!\;}^{#2}\!#1_{#3}}

%put a small hat on operators!
\providecommand{\hatop}[1]{\ensuremath{\hat{\mathop{\operator@font #1}\nolimits}}}

%A small macro for generating uppercased letters of specific math font (mathfrak).
\let\op@format\mathfrak
%\let\op@format\mathcal
\def\op#1{%
 \ifnum`#1=\lccode`#1
  \expandafter\ensuremath\op@format{\uppercase{#1}}
 \else%
  \expandafter\ensuremath\op@format{#1}
 \fi%
}%
% Jacobi elliptic functions as operators
\DeclareMathOperator{\jsn}{sn} % to replace duplicates above!
\DeclareMathOperator{\jcn}{cn}
\DeclareMathOperator{\jdn}{dn}
\DeclareMathOperator{\jns}{ns} % 1/sn(u)
\DeclareMathOperator{\jnc}{nc} % 1/cn(u)
\DeclareMathOperator{\jnd}{nd} % 1/dn(u)
\DeclareMathOperator{\jsc}{sc} % sn(u)/cn(u)
\DeclareMathOperator{\jsd}{sd} % sn(u)/dn(u)
\DeclareMathOperator{\jdc}{dc} % dn(u)/cn(u)
\DeclareMathOperator{\jds}{ds} % dn(u)/sn(u)
\DeclareMathOperator{\jcs}{cs} % cn(u)/sn(u) 
\DeclareMathOperator{\jcd}{cd} % cn(u)/dn(u)

